One Tree to Rule Them All: Poly-Logarithmic Universal Steiner Tree

A spanning tree $T$ of graph $G$ is a $\rho$-approximate universal Steiner tree (UST) for root vertex $r$ if, for any subset of vertices $S$ containing $r$, the cost of the minimal subgraph of $T$ connecting $S$ is within a $\rho$ factor of the minimum cost tree connecting $S$ in $G$. Busch et al. (FOCS 2012) showed that every graph admits $2^{O(\sqrt{\log n})}$-approximate USTs by showing that USTs are equivalent to strong sparse partition hierarchies (up to poly-logs). Further, they posed poly-logarithmic USTs and strong sparse partition hierarchies as open questions. We settle these open questions by giving polynomial-time algorithms for computing both $O(\log ^ 7 n)$-approximate USTs and poly-logarithmic strong sparse partition hierarchies. For graphs with constant doubling dimension or constant pathwidth we improve this to $O(\log n)$-approximate USTs and $O(1)$ strong sparse partition hierarchies. Our doubling dimension result is tight up to second order terms. We reduce the existence of these objects to the previously studied cluster aggregation problem and what we call dangling nets.

==> ellisScrap.tex <==
\section{Old Intro}

The past several decades have seen a remarkable development in various ways of efficiently decomposing and extracting structure from graphs and metrics with numerous applications, especially in parallel and distributed computing. Notably among these are network decompositions, ball carvings, low-diameter decompositions (LDDs), network decompositions, padded decompositions, sparse neighborhood covers, and strong graph partitions \cite{linial1993low,forster2019dynamic,blelloch2011near,awerbuch1992low,filtser2019strong, becker2019low,fox2010decompositions,elkin2022deterministic,awerbuch1996fast,abraham2008nearly,chang2021strong,bartal2004graph,kamma2017metric,rozhovn2020polylogarithmic}. Generally speaking, these constructions all separate a graph into clusters of nearby vertices while mostly respecting the structure of the distances in the graph. 

One such decomposition is a \emph{$(\alpha, \tau)$-strong partition} \cite{filtser20,jia2005universal,busch2012split}, defined as follows.\atodo{The partition are called sparse partition by previous works. I think we should keep previous notation. See \Cref{sec:oldIntro}}

% with strong diameter $\Delta$ is a partition of a graph's vertices into $\Delta$-strong-diameter clusters so that any ball of radius $\Delta / \alpha$ is incident to at most $\tau$ parts of the partition .

\begin{definition}[$\Delta$-Diameter $(\alpha, \tau)$-Sparse Strong Partitions]
	Given edge-weighted graph $G = (V, E, w)$, an $(\alpha, \tau)$-strong partition with diameter $\Delta$ is a partition of $V$ into $V = V_1 \sqcup V_2 \sqcup \ldots$ such that:
	\begin{itemize}
		\item \textbf{Low (Strong) Diameter:} $G[V_i]$ has strong diameter at most $\Delta$ for every $i$;
		\item \textbf{Ball-Avoiding:} the ball $B(v, \frac{\Delta}{\alpha})$ intersects at most $\tau$ of the $V_i$ for every $v \in V$.
	\end{itemize}
\end{definition}

%A series of works gradually improved the sorts of parameters efficiently achievable by the aforementioned decompositions from $2^{O(\sqrt{\log n})}$ \cite{awerbuch1989network} to $O(\log n)$ \cite{MillerPX2013}. 

A breakthrough result of \citet{MillerPX2013} gave a single versatile framework for producing partitions of graphs that are poly-logarithmic-quality LDDs, padded decompositions, and strong decompositions. On the other hand, remarkably little is known about natural extensions of these sorts of decompositions to hierarchical settings. In particular, very little is known if our goal is a series of partitions of increasing diameter where each decomposition must meaningfully respect the previous decomposition. 

One notable formalization of such a hierarchy is an extension of strong decompositions to the hierarchical setting, as formalized by  by Busch et al.~\cite{busch2012split}.

%if we do not require the structure of each subsequent partition to take the previous partition into account, then we can always simply freshly compute a new partition at each level. Sometimes, such hierarchies where each level can be independently computed are useful, see e.g.\ Bartal trees \cite{bartal1998approximating}.

%However, often we require that each subsequent partition is genuinely hierarchical in the sense that it must somehow respect the structure of the previous partition. For example, the following extension of ball-avoiding partitions to the hierarchical setting was introduced by \cite{busch2012split} and formalizes the requirement that each subsequent partition ``coarsens'' the previous partition.
\begin{definition}[$\gamma$-Hierarchy of $(\alpha, \tau)$-Strong Partitions]
	Given graph $G = (V, E)$, a $\gamma$-hierarchy of $(\alpha, \tau)$-strong partitions consists of partitions $\{ \{v\} : v \in V\} = \mathcal{V}_1, \mathcal{V}_2, \ldots, \mathcal{V}_k = \{\{V\}\}$ such that 
\begin{itemize}
		\item \textbf{Strong Partitions:} each $\mathcal{V}_i$ is an $(\alpha, \tau)$-strong partition with string diameter $\gamma^i$;
		\item \textbf{Coarsening:} $\mathcal{V}_{i+1}$ coarsens $\mathcal{V}_{i}$, i.e.\ if $V_{i + 1} \in \mathcal{V}_{i+1}$ then $\exists \mathcal{V}_i' \subseteq \mathcal{V}_i$ s.t.\ $V_{i + 1} = \bigsqcup_{U \in \mathcal{V}_i'} U$.
	\end{itemize}
\end{definition}
\noindent Observe that if we did not enforce the above coarsening property we could trivially compute the above partitions with poly-logarithmic parameters by applying the results of \citet{MillerPX2013}. However, the coarsening property renders computing such hierarchies highly non-trivial. \enote{A motivating difficult example / figure of a star-type thing}

Previous work has demonstrated that these hierarchies can serve as the foundation of remarkably powerful algorithmic result. For example, Busch et al.~\cite{busch2012split} demonstrated an important connection between these hierarchies and universal Steiner trees (USTs), defined as follows.

\begin{definition}[$\rho$-Approximate Universal Steiner Tree]
Given edge-weighted graph $G = (V, E, w)$, a $\rho$-approximate universal Steiner tree $T$ is a spanning tree of $G$ such that $w(T(S)) \leq \rho \cdot w(T^*_S)$ for every $S \subset V$, where $T(S)$ is the minimal subtree of $T$ connecting $S$ and $T^*_S$ is the minimum weight tree connecting $S$.
\end{definition}	
\noindent Busch et al.~\cite{busch2012split} showed that the existence of and poly-time algorithms for $\gamma$-hierarchies of $(\alpha, \tau)$-strong partitions imply the existence of and poly-time algorithms for an $O(\alpha^2\tau^2 \gamma \log n)$-approximate UST. Thus, strong partition hierarchies are a fundamental graph  decomposition with strong algorithmic implications.

However, while (non-hierarchical) strong partitions are possible with $\alpha = \tau = O(\log n)$ \cite{MillerPX2013}, in the hierarchical setting the best known bounds for general graphs are $\gamma = \alpha = \tau = 2^{O(\sqrt{\log n})}$, as proven more than 10 years ago by \citet{busch2012split}. Likewise, when combined with the above connection to USTs, this result proves the existence of $2^{O(\sqrt{\log n} \cdot \log \log n ) }$-approximate USTs which is the best known approximation factor for a UST.

 Thus, there is a nearly exponential gap between known bounds for a ``one-level'' and a hierarchical version of well-studied graph decompositions. For this reason \citet{busch2012split} posed the existence of hierarchical strong partitions with $\gamma = \alpha = \tau = \text{poly}(\log n)$ an open question.

\subsection{Our Contributions}

In this work we settle the above open question of \citet{busch2012split} by demonstrating the existence of and algorithms for strong partition hierarchies with poly-logarithmic parameterizations.

\begin{restatable}{theorem}{hierarchyThm}\label{thm:hierarchies}
    Every edge-weighted graph $G = (V,E, w)$ admits a $\gamma$-hierarchy of $(\alpha, \tau)$-strong partitions for $\gamma = BLAH$, $\alpha = BLAH$, and $\tau = BLAH$. Furthermore, this partition can be computed deterministically in polynomial time.
\end{restatable}

By extension, we demonstrate the existence of and algorithms for the first poly-logarithmic USTs.
\begin{restatable}{theorem}{USTThm}\label{thm:USTs}
    Every edge-weighted graph $G = (V,E, w)$ admits an $O(\log ^ 7 n)$-approximate universal Steiner tree. Furthermore, this tree can be computed in polynomial time.
\end{restatable}
\noindent As noted above, the previous best bounds were $\gamma = \alpha = \tau = 2^{O(\sqrt{\log n})}$ for partition hierarchies and $2^{O(\sqrt{\log n})}$-approximate universal Steiner tree. For the special case of minor-free graphs \citet{busch2012split} gave hierarchies of quality $\gamma = O(\log ^ 3 n)$, $\alpha = O(\log ^ 4 n)$ and $\tau = O(\log ^ 3 n)$ and  $O(\log ^{18} n)$-approximate universal Steiner trees and so our bounds for general graphs are an improvement over the best bounds for even the minor-free case.

We show the existence of our poly-logarithmic hierarchies by showing that, up to poly-logarithmic factors, the existence of such hierarchies is essentially equivalent to the quality of the best ``cluster aggregation'' solutions admitted by a graph. Informally, cluster aggregation aims to take a vertex partition and a collection of portal vertices and coarsen it to a partititon with one portal in each part while guaranteeing that the one portal in each vertex's coarsened cluster is nearly as close as its closest portal. Crucially for our purposes, this problem aims to provide \emph{additive} guarantees.

\begin{definition}[Cluster Aggregation]
    An instance of cluster aggregation consists of an edge-weighted graph $G = (V, E, w)$, a partition of $V$ into $\delta$ strong diameter sets $\{V_i\}_i$ and a set of portals $P \subseteq V$ where $|V_i \cap P| \leq 1$ for every $i$. A $\beta$-quality cluster aggregation solution is a partition $V = V_1' \sqcup V_2' \sqcup \ldots \sqcup V_{|P|}'$ such that and
    \begin{itemize}
        \item \textbf{Coarsening:} for each $V_j'$ we have $V_j' = \bigsqcup_{V_i \in \mcV_i}$ for some $\mcV_i \subseteq \{V_i\}_i$;
        \item \textbf{One Portal Per Cluster:} $|V_i' \cap P| = 1$ for every $i$;
        \item \textbf{$\beta$-Quality:} $d_{G[V_i']}(u, P) \leq \beta \cdot \delta  + d_G(u, P)$ for every $V_i'$ and $u \in V_i'$.
    \end{itemize}
\end{definition}
\noindent Observe that we trivially have that $\beta \geq 1$ by \enote{add path example}.

We reduce hierarchies of strong partitions to good cluster aggregation solutions.
\begin{restatable}{lemma}{CAReduction}\label{lem:red}
    Suppose graph  $G = (V, E, w)$ admits a $\beta$-quality solution for every instance of cluster aggregation. Then $G$ has a $\gamma$-hierarchy of $(\alpha, \tau)$-strong partitions for PARAMETERS.
\end{restatable}

Motivated by the above connection we further develop the algorithmics of cluster aggregation. \citet{busch2012split} previously demonstrated that all graphs admit cluster aggregation solutions of quality $O(\log ^ 2 n)$. We improve this to $O(\log n)$ which when combined with \Cref{lem:red} gives our hierarchies (\Cref{thm:hierarchies}) and universal Steiner trees (\Cref{thm:USTs}). Complementing our upper bound for cluster aggregation, we prove the (near)-optimality of this result by providing an $\Omega(\frac{\log}{ \log \log n})$ lower bound for cluster aggregation.

Lastly, we demonstrate that improved results are possible for many structured families of graphs. Specifically, we show that bounded path-width, bounded doubling dimension all admit $O(1)$ cluster aggregation solutions, leading to hierarchies of strong partitions and USTs with improved (poly-logarithmic) parameterizations on all such graphs.


==> hierarchical.tex <==
\section{Hierarchical strong partitions}

Given a partition $\mathcal{C}_{i-1}$ of clusters with strong diameter
$\rho_{i-1}$, we construct a coarsening partition ${\cal C}_{i}$
of strong diameter $\rho_{i}=O(\log^{2}n)\cdot\rho_{i-1}$ such that
every ball of radius $O(\frac{\rho_{i}}{\log n})$ will intersect
at most $O(\log n)$ clusters of ${\cal C}_{i}$. The following theorem
follows:
\begin{theorem}
	Every weighted $n$-vertex graph admits an $\left(O(\log n),O(\log n),O(\log^{2}n)\right)$-partition
	hierarchy with strong diameter.
\end{theorem}

By the general reduction in {[}BDR+12{]}, we obtain:
\begin{theorem}
	Every weighted $n$-vertex graph admits an $O(\log^{7}n)$-stretch
	UST as a subgraph.
\end{theorem}

Note that previously the state of the are by {[}BDR+12{]} was $2^{O(\sqrt{\log n})}$
for general graphs, and $O(\log^{18}n)$ for planar graphs. Thus we
answered an open question from {[}BDR+12{]} (repeated in {[}Fil20Scattering{]}).

\subsection{Algorithm}

Following {[}Fil20Scattering{]} (and using the notation from there),
we run MPX with parameter $\Delta=O(\log^{2}n)\cdot\rho_{i-1}$ with
all the vertices being centers. Following {[}Fil20Scattering{]} analysis,
we will assume that every vertex $v\in V$ got a shift $\delta_{v}\in[0,\Delta]$,
such that if $t_{v}$ is the winner, the number of vertices $u\in V$
with $f_{v}(u)=\delta_{u}-d_{G}(u,v)$ greater than $f_{v}(t_{v})-\alpha\cdot\frac{\Delta}{\log n}$
(for some universal constant $\alpha$) is bounded:
\[
\left|\left\{ u\in V\mid f_{v}(u)\ge f_{v}(t_{v})-\alpha\cdot\frac{\Delta}{\log n}\right\} \right|\le O(\log n)\,.
\]
Denote this set of vertices by $K_{v}$. Next we construct an auxiliary
graph $G'$ by adding $n$ new vertices, where for each vertex $v\in V$,
we add a new vertex $v'$ with a single edge towards $v$ of weight
$\Delta-\delta_{v}$. Denote the new vertices by $V'$, which we will
also call terminals. Note that for every pair of vertices $u,v$
\[
d_{G'}(v,u')=d_{G}(v,u)+\Delta-\delta_{u}=\Delta-f_{v}(u)\,.
\]
Hence the closest terminal to $v$ is $t'_{v}$. Furthermore, there
are at most $O(\log n)$ terminals, at distance at most $d_{G'}(u,t'_{v})+\alpha\cdot\frac{\Delta}{\log n}$
from $v$. Denote these terminals by $K'_{v}$.

Next we use a cluster aggregation algorithm w.r.t. ${\cal C}_{i-1}$
(the terminals are just the auxiliary singletons), as a result we
obtain a function $g:V\cup V'\rightarrow V'$ which is consistent
on ${\cal C}_{i-1}$, and where each vertex $v$ is sent to a terminal
at distance at most $d_{G'}(v,t'_{v})+\beta\cdot\log n\cdot\rho_{i-1}$
for some universal constant $\beta$ (note- this is a bound on the
distance in the induced graph by the cluster). The final clusters
we return will by the clusters returned by the cluster aggregation
algorithm (after removing the terminals).

\subsection{Analysis}

First we bound the diameter of every cluster in $G'$. As each vertex
$v$ is sent to a terminal at distance at most $\Delta-f_{v}(t{}_{v})+\beta\cdot\log n\cdot\rho_{i-1}$,
clearly, the diameter of each cluster is bounded by
\[
\rho_{i}=2\Delta+2\beta\cdot\log n\cdot\rho_{i-1}<3\Delta\,.
\]
Clearly this bounds hold in the graph without the terminals as well. 

Next, consider a ball around $v$ of radius $R=O(\frac{\Delta}{\log n})=O(\frac{\rho_{i}}{\log n})$.
For every $u\in B_{G}(v,r)$, $u$ is sent to some terminal $t'$.
Let $t_{u}$ be the winner of the MPX for $u$. It holds that
\[
f_{u}(t{}_{u})\ge f_{u}(t{}_{v})=\delta_{t_{v}}-d_{G}(u,t_{v})\ge\delta_{t_{v}}-d_{G}(v,t_{v})-d_{G}(u,v)=f_{v}(t{}_{v})-d_{G}(u,v)\,.
\]
By the cluster aggregation property we have that 
\begin{align*}
	d_{G'}(v,t') & \le d_{G'}(v,u)+d_{G'}(u,t')\\
	& \le d_{G}(v,u)+\Delta-f_{u}(t{}_{u})+\beta\cdot\log n\cdot\rho_{i-1}\\
	& \le2\cdot d_{G}(v,u)+\Delta-f_{v}(t{}_{v})+\beta\cdot\log n\cdot\rho_{i-1}\\
	& \le d_{G'}(v,t'_{v})+2R+\beta\cdot\log n\cdot\rho_{i-1}\\
	& \le d_{G'}(v,t'_{v})+\alpha\cdot\frac{\Delta}{\log n}\,.
\end{align*}
For an appropriate choice of $R$, and large enough constant in the
definition of $\Delta$. It follows that $t'\in K'_{v}$. In particular,
all the vertices in $B_{G}(v,R)$ are clustered to terminals in $K_{v}$.
As there are only $O(\log n)$ terminals in $K_{v}$, our analysis
is concluded.


==> oldVersions/CADanielOriginal.tex <==
%
%\begin{comment}
%
%
%\subsection{General Graphs - original}
%
%We begin by demonstrating how to achieve $O(\log N)$-distortion cluster aggregation solutions in general graphs when we are given $N \leq n$ input clusters.
%\CAGeneral*
%
%\noindent Our main approach is to grow the cluster of each portal in a round-robin and geometric fashion but treat each vertex's path to its nearest cluster with a portal as having length $0$; this idea is generally in the spirit of the star decompositions of \cite{dhamdhere2006improved} (see also the related Relaxed Voronoi algorithm \cite{Fil19sicomp}).
%
%\dtodoin{First draft of cluster aggregation in general graphs. Need to fix notation to be consistent with intro.}
%
%
%To formalize this, for each cluster $V_i \in \mc{V}$, arbitrarily choose a representative vertex $v_i \in V_i$, and let $F_i$ denote a shortest path in $G$ from $v_i$ to its closest portal. When we say a prefix $F_i'$ of $F_i$ is \textit{internally disjoint} from some clusters, we mean it is node-disjoint in all but the final node of the prefix, which we denote by $\final(F_i')$. 
%
%\paragraph*{Algorithm Overview} Order the portals arbitrarily $p_1, \ldots, p_L$, and proceed in rounds. In every round $j$, each portal $p_\ell$ in sequence expands $V_\ell'$, the set of clusters assigned to it, by claiming \textit{all} clusters used by any of the representative shortest paths entering $V_\ell'$, the \textit{frontier paths} $\mc{F}_{\ell h}^{(j)}$. Portal $p_\ell$ repeats this expansion a geometric variable $g_\ell^{(j)}$-many times, then we move on to the next portal. Clearly each $Q_\ell$ remains connected. We will show that only $O(\log(\abs{\mc{V}}))$ rounds are needed to assign every cluster to a portal, and that the total detour of a node assigned to any portal $p_\ell$ is at most $2\Delta \cdot \sum_j g_\ell^{(j)}$, which will suffice to prove the theorem. The algorithm is presented formally in \Cref{alg:cluster-agg-general}.
%
%\atodoin{Perhaps better to abuse notation and send clusters to portals}
%\dtodoin{As in, replace the notation of $V_\ell'$ with $f^{-1}(p_\ell)$? I can do this if it seems better.}
%
%\begin{algorithm}[h]
%\caption{\texttt{Cluster aggregation for general graphs}}
%\label{alg:cluster-agg-general}
%\DontPrintSemicolon
%\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%\Input{weighted $G = (V, E,w)$, portal set $P \subseteq V$, partition $\mc{V} = \{V_i\}_i$ into clusters of strong diameter at most $\Delta$.}
%\Output{an assignment $f: \mc{V} \to P$ of additive	 distortion $\beta = O(\log\abs{\mc{V}})$.}
%\BlankLine
%
%Name the portals $P = \{p_1, \ldots, p_L\}$\; 
%
%For each $p_\ell$ contained in cluster $V_i$, initialize the clusters assigned to $p_\ell$ as $V_\ell' \gets \{V_i\}$\;
%
%\For{rounds $j = 1, 2, \ldots, 10\log\abs{\mc{V}}$}{
%\For{portals $p_\ell = p_1, \ldots, p_L$}{
%Draw $g_{\ell}^{(j)} \sim \text{Geom}(\frac{1}{10})$\;
%\For{$\text{h} = 1, \ldots, g_\ell^{(j)}$ (expansion iterations)}{
%Let $\mc{U} = \mc{V} \setminus \bigcup_{\ell'} V_{\ell'}'$ be the unassigned clusters\;
%For each $V_i \in \mc{U}$, let $F_i'$ be the maximal prefix of $F_i$ internally disjoint from all assigned clusters\;
%
%Consider the frontier paths $\mc{F}^{(j)}_{\ell h} = \{F_i' \mid \text{final}(F_i') \in V_\ell'\}$\;
%
%Update $V_\ell' \gets V_\ell' \cup \{V_i \in \mc{U} \mid V_i \cap F_{i'}' \neq \varnothing \text{ for some frontier path } F_{i'}' \in \mc{F}^{(j)}_{\ell h}\}$\;
%}
%}
%}
%Assign each cluster in $V_\ell'$ to $p_\ell$ for each $\ell$\;	
%\end{algorithm}
%\atodoin{$Q_i$ in the pseudo code is undefined}
%
%\begin{lemma}
%\label{lem:assignment-whp}
%The algorithm assigns every cluster, with high probability.\atodo{quantify}
%\end{lemma}
%\begin{proof}
%We claim that in each round $j$, an unassigned cluster $V_i$ has probability at least $\frac{9}{10}$ of being assigned to a portal. Consider the prefix $F_i'$ of $F_i$ internally disjoint from assigned clusters at the beginning of round $j$, and let $p_{\ell^*}$ be the portal for which $\final(F_i') \in V_{\ell^*}'$. Consider the event $A_{V_i, j}$ that there is some $\ell < \ell^*$ for which $p_\ell$ claims a cluster used by $F_i'$ in round $j$.
%\begin{itemize}
%\item If event $A_{V_i,j}$ does not occur, then $F_i'$ is a frontier path for $p_{\ell^*}$ in its first expansion: $F_i' \in \mc{F}^{(j)}_{\ell^*1}$, so $\Pr[V_i \text{ assigned to } p_{\ell^*} \mid \neg A_{V_i, j}] = 1$. 
%
%\item Otherwise, let $\ell'$ be the least $\ell < \ell^*$ for which $p_{\ell}$ claims a cluster used by $F_i'$, and let $h$ be the expansion iteration for $p_{\ell'}$ at which this first occurs. Then some prefix of $F_i'$ becomes a frontier path for $p_{\ell'}$ after expansion $h$, and since $g_{\ell'}^{(j)}$ is geometrically distributed, we have
%\[
%\Pr\left[V_i \text{ assigned to } p_{\ell'} \mid A_{V_i, j}\right] = \Pr\left[g_{\ell'}^{(j)} \geq h + 1 \Bigm\vert g_{\ell'}^{(j)} \geq h\right] = \frac{9}{10}.
%\]
%\end{itemize}
%So by the law of total probability it follows that $\Pr[V_i \text{ assigned in round } j] \geq \frac{9}{10}$. Furthermore, while the rounds are not necessarily independent, it is clear this bound holds for any unassigned cluster in round $j$ conditioned on any events that depend only on previous rounds. Therefore, denoting by $B_{V_i, j}$ the event that cluster $V_i$ is \textit{not} assigned in round $j$, we have
%\[
%\Pr[V_i \text{ not assigned}] = \Pr\Bigg[\bigcap_{j} B_{V_i, j}\Bigg] = \prod_{j} \Pr\left[B_{V_i, j} \mid B_{V_i, 1}, \ldots, B_{V_i, j-1}\right] \leq \left(\frac{1}{10}\right)^{10\log\abs{\mc{V}}} \leq \frac{1}{\abs{\mc{V}}^{10}}.
%\]
%Taking a union bound over $\mc{V}$ yields the desired result. 
%\atodo{Taking geometric distribution with $p=\frac12$ will be enough for this argument. Why $\frac{1}{10}$?}
%\end{proof}
%
%\begin{theorem}\atodo{Theorem without a label. Should be stated at the start of the section}
%The algorithm produces an assignment with detour $\dtr_f \leq O(\log \abs{\mc{V}}) \cdot \Delta$, with high probability. 
%
%\begin{proof}
%We claim that in any round $j$, a cluster $V_i$ assigned to some $p_\ell$ in its $h$th iteration of expansion satisfies (recall $v_i \in V_i$ is the representative for $V_i$)
%\begin{equation}\label{eq:cluster-agg-induction}
%d_{G[V_\ell']}(v_i, p_\ell)\leq d_G(v_i, P) + 4\left(1+ \sum_{j' = 1}^{j - 1} g_\ell^{(j')} + h\right) \cdot \Delta 
%\end{equation}
%We prove this by induction. When $j = 0$, all $V_\ell'$ are initialized to contain only the cluster $V_i$ in which portal $p_\ell$ lies, so $d_{G[V_\ell']}(v_i, p_\ell) \leq \Delta \leq d(v_i, P) + 4\Delta$. 
%
%For any $j \geq 1$, consider some cluster $V_i$ claimed by portal $p_\ell$ during round $j$ after $h$ expansion iterations. This means there was some frontier path $F'_{i'} \in \mc{F}_{\ell h}^{(j)}$ entering $V_\ell'$ and intersecting $V_i$. Say $F'_{i'}$ enters $V_\ell'$ at node $u$, contained in some cluster $V_{i^*}$, and leaves cluster $V_i$ at node $w$. We will denote the segment of $F'_{i'}$ from $w$ to $u$ as $F'_{i'}[w:u]$, and similarly for other segments. See \Cref{fig:genCA} for an illustration. 
%\begin{figure}[h]
%\centering
%\centering        \includegraphics[width=0.5\columnwidth,trim=0mm 170mm 0mm 0mm, clip]{figures/genCA.pdf}
%\caption{The paths involved in bounding $d_{G[V_\ell']}(v_i, p_\ell)$. The blue path $F'_{i'}$ is the frontier path that caused $V_i$ to be assigned to $p_\ell$; the yellow paths are shortest paths within a cluster, so have length at most $\Delta$; and the red path is a shortest path within the coarsened cluster $V_\ell'$, so its length is bounded by the induction hypothesis.}\label{fig:genCA}
%\end{figure}
%\atodoin{The figure is referenced nowhere. It is also will be better if the shortest path will be more of a straight line, and perhaps if we show at least 2 steps of expansion (i.e. the difference between $g_\ell^(j)=1$ and $g_\ell^(j)=2$)}
%\noindent Now observe that after the $h$th expansion, we have a path in $V_\ell'$ from $v_i$ to $p_\ell$:
%\[
%d_{G[V_\ell']}(v_i, p_\ell) \leq d_{G[V_i]}(v_i, w) + \abs{F'_{i'}[w:u]} + d_{G[V_{i^*}]}(u, v_{i^*}) + d_{G[V_\ell']}(v_{i^*}, p_\ell)
%\]
%since the entirety of $F_{i'}' = F_{i'}'[v_{i'}:u]$ is now contained in $V_\ell'$. The first and third terms are clearly bounded by $\Delta$. Now, since $V_{i^*}$ must have been assigned to $p_\ell$ at some earlier expansion iteration or round, we apply the induction hypothesis for round $j$ with $h-1$ expansion iterations:
%\begin{align*}
%d_{G[V_\ell']}(v_i, p_\ell) &\leq 2\Delta + \abs{F'_{i'}[w:u]} + d_G(v_{i^*}, P) + 4\biggl(1+ \sum_{j' = 1}^{j - 1} g_\ell^{(j')} + (h-1)\biggr) \cdot \Delta \\
%&\leq 2\Delta + \abs{F'_{i'}[w:u]} + (\underbrace{d_G(u, P)}_{=\abs{F_{i'}[u:]}} + \Delta) + 4\biggl(1+ \sum_{j' = 1}^{j - 1} g_\ell^{(j')} + (h-1)\biggr) \cdot \Delta \\
%&= 3\Delta + \underbrace{\abs{F_{i'}[w:]}}_{=d_G(w, P)} + 4\biggl(1+ \sum_{j' = 1}^{j - 1} g_\ell^{(j')} + (h-1)\biggr) \cdot \Delta\\
%&\leq 3\Delta + (d_G(v_i, P) + \Delta) + 4\biggl(1+ \sum_{j' = 1}^{j - 1} g_\ell^{(j')} + (h-1)\biggr) \cdot \Delta\\
%&= d_G(v_i, P) + 4\biggl(1+ \sum_{j' = 1}^{j - 1} g_\ell^{(j')} + h\biggr) \cdot \Delta
%\end{align*}
%as desired.
%
%With the claim proved, we get that at the end of the algorithm that every representative $v_i$ of a cluster assigned to $p_\ell$ satisfies $d_{G[V_\ell']}(v_i,p_\ell) - d_G(v_i, P) \leq 4(1 + \sum_{j'=1}^{10\log\abs{\mc{V}}} g_\ell^{(j')}) \cdot \Delta$. Letting $X \sim \text{Bin}(200\log\abs{\mc{V}}, \frac{1}{10})$, we have for any sum of IID geometric random variables
%\[
%\Pr\left[\sum_{j'=1}^{10\log|{\cal V}|}g_{\ell}^{(j')}>200\log|{\cal V}|\right]=\Pr\left[X<10\log|{\cal V}|\right]=\Pr\left[X<\frac{1}{2}
%\mathbb{E}
%\left[X\right]\right]
%<e^{-\mathbb{E}
%\left[X\right]/8}\leq\frac{1}{|{\cal V}|^{2}}
%\]
%by a standard Chernoff bound. Then, a union bound over $\mc{V}$ shows that the algorithm produces an assignment with detour $\leq (1 + 200\log \abs{\cal V}) \cdot \Delta$ for every assigned representative, and therefore an assignment with detour $\leq (2 + 200\log \abs{\cal V}) \cdot \Delta$ for every node in an assigned cluster, with high probability. Finally, letting $B_{U}$ denote the event that there is an unassigned cluster, and $B_R$ the even that some assigned representative has detour $> (1 + 200\log \abs{V}) \cdot \Delta$, we have by \cref{lem:assignment-whp} and a union bound:
%\[
%\Pr[\dtr_f > (2 + 200\log \abs{\cal V}) \cdot \Delta] \leq \Pr[B_U] + \Pr[B_R] \leq \frac{1}{\abs{\mc{V}}^{9}} + \frac{1}{\abs{\mc{V}}} \leq \frac{2}{\abs{\mc{V}}} \qedhere
%\]
%\end{proof}
%\end{theorem}
%
%\end{comment}



==> oldVersions/OldMPXBasedProof.tex <==

\todo[inline]{Original proof, MPX based}


\begin{definition}[$(\alpha,\tau,\Delta)$-MPX based partition]
	Given a weighted graph $G=(V,E,w)$, a set of centers $N\subseteq V$, and a collections of shifts $\{\delta_t\}_{t\in N}$, a partition $\calC=\{C_t\}_{t\in N}$ of the vertices is well defined. We say that $\calC$ is $(\alpha,\tau,\Delta)$-MPX based partition if the following hold:
	\begin{itemize}
		\item The strong diameter of every cluster $C_t\in\calC$ is at most $\Delta$. In particular, $\max_{t\in N}\delta_t\le\frac\Delta2$, and for every $t\in N$ and $v\in C_t$ it holds that $d_{G[C_t]}(t,v)\le\frac\Delta2$.
		\item Every ball of radius $\frac\Delta\alpha$ intersects at most $\tau$ clusters. Furthermore, for every vertex $v$, let $t_v$ be the center clustering $v$: $t_v=\argmax_{t\in N} f_v(t)$. The number of centers $t$ with margin of loss $\frac{2\Delta}{\alpha}$ is at most $\tau$: $\left|\left\{t\mid f_v(t)\ge f_v(t_v)-\frac{2\Delta}{\alpha}\right\}\right|\le\tau$.
	\end{itemize}
\end{definition}

\subsection{Hierarchical Strong Sparse Partition}


\begin{restatable}{theorem}{CAReduction2}\label{thm:MetaHierarchicalMPXBased}
	Consider a weighted graph  $G = (V, E, w)$, such that:
	\begin{itemize}
		\item For every $\Delta>0$, $G$ has a $(\eps,\tau,\Delta)$-auxiliary graph $G'$ (with set $N\subseteq V$) that induces an $(\alpha,\tau,\Delta)$-Voronoi based partition.
            \item For every $(\eps,\tau,\Delta)$-auxiliary  graph $G'$, there is a $\beta$-distortion solution for every instance of cluster aggregation  of $G'$ with $N'$ as portals. 
	\end{itemize} 
	Then $G$ has a $\rho =2\beta\cdot\left(\alpha+1\right)$-hierarchy of strong $(4(\alpha+1),\tau)$-sparse partitions. Furthermore, if each MPX based partition, and cluster aggregation instance can be solved in polynomial time then the hierarchy can be computed in polynomial time.
\end{restatable}

We now describe the algorithm for strong sparse partition hierarchies
using cluster aggregation.  
Our algorithm proceeds in rounds in a bottom up fashion, with round $0$ being the construction of a strong sparse partition ${\cal C}_0$, and round $i$ constructing the coarsening of strong sparse
partition ${\cal C}_{i-1}$ to obtain strong sparse partition ${\cal
  C}_i$.  In the remainder, we elaborate on the coarsening step of
round $i$.

Here we receive as input an $(2(\alpha+1),\tau,\rho^{i-1})$-strong sparse partition $\calC_{i-1}$.
Let $\Delta=2\alpha\beta\cdot\rho^{i-1}$.
Using the assumption, we create an $(\alpha,\tau,\Delta)$-MPX based partition $\calC_{\sMPX}$ of $G$.
Specifically, we obtain a subset $N\subseteq V$ of centers and a collections of shifts $\{\delta_t\}_{t\in N}$ such that  $\calC_{\sMPX}=\{C_t\}_{t\in N}$ where $v$ joins the cluster $t_v=\argmax_{t\in N} f_v(t)=\argmax_{t\in N} \delta_t-d_G(v,t)$. In particular, for every $v\in V$ it holds that $\left|\left\{t\mid f_v(t)\ge f_v(t_v)-\frac{2\Delta}{\alpha}\right\}\right|\le\tau$.

Next we construct an auxiliary graph $G'$ by adding  new auxiliary vertices $N'=\{t'\mid t\in N\}$. 
For each vertex $t\in N$, we add a new vertex $t'$
with a single edge towards $t$ of weight $\frac\Delta2-\delta_{v}$.
%Denote the auxiliary vertices by $V'$.
%
Next apply the cluster aggregation algorithm in the auxilery graph $G'$ w.r.t. to clusters ${\cal C}_{i-1}$ and the portal set $N'$ (the portals themselves are considered singleton clusters).
As a result we obtain a function $g:V\cup N'\rightarrow N'$ which is consistent on ${\cal C}_{i-1}$, and where each vertex $v$ is sent to a portal $g(v)$ at distance
at most $d_{G'[g^{-1}(g(v))]}(v,g(v))\le d_{G'}(v,N') +\beta\cdot\rho_{i-1}$. The final clusters we return
will simply be $\left\{g^{-1}(t')\setminus\{t'\}\right\}_{t\in N}$
the clusters returned by the cluster aggregation algorithm
(after removing the auxiliary vertices).  The algorithm is formally
presented below.

\begin{algorithm}[h]	
    \begin{algorithmic}[1]
    	\caption{\texttt{Hierarchical-Strong-Sparse- Partition}}\label{alg:HierarchicalMPXbased}
        \Require Weighted graph $G = (V,E,w)$ (with all weight being at least $1$),
        algorithm producing $(\alpha,\tau,\cdot)$-MPX based partitions for $G$, algorithm 
        producing $\beta$-distortion solution for every instance of cluster aggregation on auxilery graphs of $G$.         
        \Ensure $\rho=2\beta\cdot\left(\alpha+1\right)$-hierarchy of strong $(4(\alpha+1),\tau,\rho)$-sparse partitions.
%        $\gamma$-hierarchy of strong $(\alpha, \tau)$-partitions $\{{\cal C}_i\}$.
		\State $i=0$, and $\rho=2\beta(\alpha+1)$.
		\State Set $\calC_0=\{\{v\}\mid v\in V\}$.
		
		\While{$\calC_i\ne\{\{V\}\}$}
			\State $i\leftarrow i+1$.
			\State Set $\Delta=\alpha\beta\cdot\rho^{i-1}$.
			\State Create a $(\alpha,\tau,\Delta)$-MPX based partitions for $G$. In particular let $N\subseteq V$ be the received centers with shifts $\{\delta_t\}_{t\in N}$.
			
			\State  Construct an auxiliary graph $G' = (V \cup N', E \cup E')$ where
			$N' = \{\aux{t}: t \in N\}$ and $E' = \{(t,\aux{t}): t \in N\}$ with weight of edge
			$(t, \aux{t})$ being $\frac\Delta2 - \delta_t$.
			
			\State Run Cluster Aggregation on graph $G'$ with clusters $\calC_i$ and portal
			set $N'$ to obtain partition ${\cal C}'$.
			
			\State Let ${\cal C}_{i}=\{C \setminus N'\mid C \in \calC'\}$.			
		\EndWhile
		\Return $\calC_0,\calC_1,\dots,\calC_i$.
%
%        \State Run algorithm from [Fil20Scattering] to obtain an
%        $(\alpha, tau)$-partition ${\cal C}_0$.  Let $\rho_0 = 1$.
%        
%        \For{$i = 1, 2, \ldots, $}
%             \State Run [MillerPX2013] clustering with parameter $\Delta = \lambda
%             \log^{2} n \rho_{i-1}$.  Let $\delta_v$ denote the shift of
%             $v$ and let $\win{v}$ denote the winner for $v$.
%
%             \State Construct an auxiliary graph $G' = (V \cup V', E \cup E')$ where
%             $V' = \{\aux{v}: v \in V\}$ and $E' = \{(v,\aux{v}): v \in V\}$ with weight of edge
%             $(v, \aux{v})$ being $\Delta - \delta_v$.
%
%             \State Run Cluster Aggregation on graph $G'$ with portal
%             set $V'$ to obtain partition ${\cal C}'$.
%
%             \State Let ${\cal C}_i$ denote $\{C - V': C \in {\cal C}\}$.
%        \EndFor
    \end{algorithmic}
\end{algorithm}

%We begin with an important property of [MPX] established in
%{[}Fil20Scattering{]}.  For a given vertex $v$, let $K_v$ denote the
%set of vertices $u$ in $V$ with $f_{v}(u)=\delta_{u}-d_{G}(u,v)$
%greater than $f_{v}(\win{v})-\alpha\cdot\frac{\Delta}{\log n}$ (for some
%universal constant $\alpha$).  That is,
%\[
%K_v = \left\{ u\in V\mid f_{v}(u)\ge f_{v}(t_{v})-\alpha\cdot\frac{\Delta}{\log n}\right\}.
%\]
%It is shown in {[}Fil20Scattering{]} that with high probability, the
%cardinality of $K_v$ is $O(\log n)$ for all $v \in V$.
%
%For a given vertex $v$, let $K'_v$ denote the set of portals in $G'$
%whose distance to $v$ is at most $\alpha\cdot\frac{\Delta}{\log n}$
%more than the distance of $v$ from its closest portal.
%
%\begin{lemma}
%With high probability, the cardinality of $K'_v$ is $O(\log n)$ for all
%$v \in V$.
%\end{lemma}
%\begin{proof}
%For every pair of vertices $u,v$
%\[
%d_{G'}(v,\aux{u})=d_{G}(v,u)+\Delta-\delta_{u}=\Delta-f_{v}(u)\,.
%\]
%Hence the closest portal to $v$ is $\auxwin{v}$.  Furthermore, by the
%  definition of $K_v$, if $d_{G'}(v,\aux{u})$ is at most
%  $d_{G'}(u,\auxwin{v})+\alpha\cdot\frac{\Delta}{\log n}$, then $u$ is
%  in $K_v$.  Therefore, by the upper bound on $|K_v|$ due to
%  {[}Fil20Scattering{]}, $|K'_v|$ is $O(\log n)$ with high
%  probability.
%\end{proof}

\begin{LabeledProof}{Theorem~\ref{thm:MetaHierarchicalMPXBased}}
We now establish that for every $i$, ${\cal C}_i$ forms a strong $\rho^i$-diameter $(\alpha, \tau)$-sparse partition.  The claim holds
for $i = 0$ since ${\cal C}_0$ is a strong $\rho^0$-diameter $(4(\alpha+1),
\gamma)$-sparse partition.  

Consider arbitrary $i > 0$. We assume by induction that $\calC_{i-1}$ is a $(4(\alpha+1),\tau,\rho^{i-1})$-strong sparse partition.
Recall that $\Delta=2\alpha\beta\cdot\rho^{i-1}$.
The analysis proceeds in two parts.  We
first bound the diameter of every cluster in $\{{\cal C}_i\}$. 
Consider a vertex $v\in V$.
Initially, in the $(\alpha,\tau,\Delta)$-MPX based partition $v$ is sent to center $t\in N$ such that $d_G(t,v)\le\frac\Delta2$. Then in the auxilery graph $G'$ it holds that 
\[
d_{G'}(v,N')\le d_{G'}(v,t')=d_{G'}(v,t)+d_{G'}(t,t')\le\frac{\Delta}{2}+\frac{\Delta}{2}-\delta_{t}\le\Delta~.
\]
Next we obtained a solution $g:V'\rightarrow N'$ to the cluster aggregation problem where $v$ is sent to portal $\tilde{t}'$ such that $d_{G'[g^{-1}(\tilde{t}')]}(v,\tilde{t}')\le d_{G'}(v,N')+\beta\cdot\rho^{i-1}=\Delta+\beta\cdot\rho^{i-1}$. It follows that $v$ is contained in a cluster of strong diameter at most $2\cdot\left(\Delta+\beta\cdot\rho^{i-1}\right)=2\beta\cdot\left(\alpha+1\right)\cdot\rho^{i-1}=\rho^{i}$. Finally, In the actual partition $\calC_i$ in the cluster $g^{-1}(\tilde{t}')$ we remove the auxilery vertices from $N'$. As all this vertices are of degree $1$, the diameter of $g^{-1}(\tilde{t}')$ can only decrease. 
We conclude that $\calC_i$ has indeed strong diameter $\rho^i$ as required. It is also clear that $\calC_i$ coarsens $\calC_{i-1}$.
 
%Due to the cluster aggregation, $v$ 
%Since
%each vertex $v$ is sent to a portal at distance at most
%$\Delta-f_{v}(\win{v})+\beta\cdot\log n\cdot\rho_{i-1}$ in $G'$, the
%diameter of each cluster is bounded by
%\[
%\rho_{i}=2\Delta+2\beta\cdot\log n\cdot\rho_{i-1}<3\Delta\,.
%\]
%Clearly this bound holds in $G$ as well.

Next, we bound the ball preservation property. Fix a vertex $v\in V$, and let $t_v\in N$ be the ``winner'' of the MPX race: $t_v=\argmax_{t\in N} f_v(t)=\argmax_{t\in N} \delta_t-d_G(v,t)$.
Consider a ball around $v$ of radius $R=\frac{\Delta}{2\alpha}$.
For every $u\in B_{G}(v,R)$, $u$ is sent to some terminal $\aux{t}\in N'$ (which corresponds to $t\in N$). 
By the cluster aggregation property we have that
\begin{align*}
	d_{G'}(v,\aux{t}) & \le d_{G'}(v,u)+d_{G'}(u,\aux{t})\\
	& \le d_{G'}(v,u)+d_{G'}(u,N')+\beta\cdot\rho_{i-1}\\
	& \le d_{G'}(v,N')+2d_{G'}(v,u)+\beta\cdot\rho_{i-1}\\
	& \le d_{G}(v,t_{v})+d_{G}(t_{v},t'_{v})+\frac{\Delta}{\alpha}+\frac{\Delta}{\alpha}\\
	& =d_{G}(v,t_{v})+\frac{\Delta}{2}-\delta_{t_{v}}+\frac{2\Delta}{\alpha}\\
	& =\frac{\Delta}{2}-f_{v}(t_{v})+\frac{2\Delta}{\alpha}~,
\end{align*}
In particular, it implies that
\begin{align*}
	f_{v}(t) & =\delta_{t}-d_{G}(v,t)=\delta_{t}-\left(d_{G'}(v,t')-\left(\frac{\Delta}{2}-\delta_{t}\right)\right)\\
	& =\frac{\Delta}{2}-d_{G'}(v,t')\ge f_{v}(t_{v})-\frac{2\Delta}{\alpha}~.
\end{align*}
However, as $\left|\left\{ t\in N\mid f_{v}(t)\ge f_{v}(t_{v})-\frac{2\Delta}{\alpha}\right\} \right|\le\tau$,
it follows that the vertices in $B_{G}(v,R)$ are sent to at most
$\tau$ different clusters, as required.
Finally, the padding of the partition $\calC_i$ is
\[
\frac{\rho^{i}}{R}=\frac{\rho^{i}}{\frac{\Delta}{2\alpha}}=\frac{2\alpha\cdot\rho^{i}}{\alpha\cdot\beta\cdot\rho^{i-1}}=\frac{2\rho}{\beta}=\frac{2\cdot2\beta\cdot\left(\alpha+1\right)}{\beta}=4(\alpha+1)~,
\]
concluding our analysis and proof.


%
%
%
%\atodoin{End}
%
%
%It holds that
%We thus have
%\[
%f_{u}(\win{u})\ge f_{u}(\win{v})=\delta_{\win{v}}-d_{G}(u,\win{v})\ge\delta_{\win{v}}-d_{G}(v,\win{v})-d_{G}(u,v)=f_{v}(\win{v})-d_{G}(u,v)\,.
%\]
%By the cluster aggregation property we have that 
%\begin{align*}
%	d_{G'}(v,\aux{t}) & \le d_{G'}(v,u)+d_{G'}(u,\aux{t})\\
%	& \le d_{G}(v,u)+\Delta-f_{u}(\win{u})+\beta\cdot\log n\cdot\rho_{i-1}\\
%	& \le2\cdot d_{G}(v,u)+\Delta-f_{v}(\win{v})+\beta\cdot\log n\cdot\rho_{i-1}\\
%	& \le d_{G'}(v,\auxwin{v})+2R+\beta\cdot\log n\cdot\rho_{i-1}\\
%	& \le d_{G'}(v,\auxwin{v})+\alpha\cdot\frac{\Delta}{\log n}~,
%\end{align*}
%for an appropriate choice of $R$, and large enough constant in the
%definition of $\Delta$. It follows that $t'\in K'_{v}$. In particular,
%all the vertices in $B_{G}(v,R)$ are clustered to terminals in
%$K_{v}$.  As there are only $O(\log n)$ terminals in $K_{v}$, this
%establishes the ball preservation property, concluding our analysis
%and proof.
\end{LabeledProof}

==> oldVersions/TreeEllisOriginalProof.tex <==
\subsection{Trees}
In this section we give our $O(1)$-distortion cluster aggregation solutions for trees. The fact that trees admit constant distortion solutions is not trivial at first glance. Indeed, related structures such as strong sparse partitions in trees exhibit $\tilde{\Omega}(\log n)$ lower bounds \cite{Fil20}. 
The basic idea is to exploit the fact that all simple paths in a rooted tree have an ``up'' part and then a ``down'' part which allows us to limit the number of conflicts when trying to coarsen our partition.

We begin by describing our algorithm. Consider an instance of cluster aggregation on $G = (V,E, w)$ with portals $P \subseteq V$ and initial partition $\mcV$ of diameter $\Delta$ where $G$ is a tree.  
For simplicity we will assume that all portals are leafs, and contained in a singleton clusters.
A general instance can be reduced to this case by simply adding an auxilery portal $p'$ for each portal $p\in P$ with a single edge $(p,p')$ of weight $0$, and the singleton clusters $\{p'\}_{p\in P}$ to $\mcV$. It is east to see that a solution to the auxilery case immediately implies a solution to the original tree of the same quality. 

%We let $\tilde{P} := \{v : v \in V_i \text{ and } V_i \cap P \neq \emptyset\}$ be all vertices in a cluster in $\mcV$ containing a portal so that $P \subseteq \tilde{P}$.
Root $G$ arbitrarily at root $r \in V$. As we may assume that each part of $\mcV$ is connected,\footnote{Since otherwise quality $0$ cluster aggregation is trivial.} each part $V_i \in \mcV$ has a unique vertex $r_i$ which is closest to $r$. Likewise, let $P_i$ be the shortest path in $G$ from $r_i$ to $\tilde{P}$. Let $t_i$ be the endpoint of this path and let $p_i$ be the portal in the same cluster as $t_i$. For simplicity of presentation we assume that $P_i$ is unique. Note that $t_i$ is in a part of $\mcV$ containing $p_i$ but may not itself be a portal. 

%\enote{Re breaking ties: you have to be careful about tie breaking and always prefer e.g. monotone down paths to monotone up paths. I wrote it down with tie-breaking but it ended up being somewhat messy /distracting from the main idea imo so I instead just assumed shortest paths are unique. $t_i$ is in a cluster containing a portal but not necesarilly a portal.}
We partition the $V_i \in \mcV$ into three sets. 
\begin{itemize}
	\item \textbf{Trivial:} Say that $V_i$ is trivial part if $P_i = (r_i)$; in other words $\{p_i\} = V_i \cap P$.
	\item \textbf{Monotone:} Say that $V_i$ is 
	\emph{monotone up} if $t_i$ is an ancestor of $r_i$ in $G$, \emph{monotone down} if $t_i$ is a descendant of $r_i$ in $G$ and \emph{monotone} if it is either monotone up or monotone down.
	\item \textbf{Bitone:} Say that $V_i$ is \emph{bitone} if $t_i$ is neither an ancestor nor a descendant of $r_i$ in $G$. For a bitone part, we let $t_i'$ be the unique vertex in $P_i$ where $P_i$ switches from ``going up'' to ``going down''; that is, $t_i'$ is an ancestor of all vertices of $P_i$ in $G$.
\end{itemize}
\noindent Additionally, we say that a part $V_i$ is \emph{reflective} if there is a bitone part $V_j$ such that $V_i$ contains $t_j'$. 

We now construct our cluster aggregation solution $\mcV'$ as follows. See \Cref{fig:treeAlg} for an illustration. \atodoin{Perhaps add all this name into the figure. I am still confused about how it can be that $p_i\ne t_i$.} \enote{Which name?}
\atodoin{The names from the definitions above for a better illustratoin. $p_i,t_i,t'_j,V_i$ etc.}


\begin{enumerate}
	\item \textbf{Assign Trivial Parts:} For each trivial part $V_i$, we assign $V_i$ to the one portal in $V_i$. That is, we let $f(V_i) = p_i$. 
	\item \textbf{Assign Monotone Parts:} Next, we cluster each monotone $V_i$ with its preferred cluster; that is, we also let $f(V_i) = p_i$ for each monotone $V_i$.
	
	\item \textbf{Assign Reflective Bitone Parts:} For each reflective bitone part $V_i$ containing a $t_j'$ we  assign $V_i$ to $V_j$'s preferred portal, namely $f(V_i) = p_j$. If there are multiple such $V_j$ we pick an arbitrary one. 
	\item  \textbf{Assign Non-Reflective Bitone Parts:} For each so far unassigned bitone part $V_i \in \mcV$, let $V_j$ be the unique cluster containing $t_i'$. In this case, $V_i$ joins the part to which $V_j$ was already assigned; that is, we let $f(V_i) = f(V_j)$.
\end{enumerate}

\begin{figure}[h]
	\centering
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[width=\textwidth,trim=0mm 0mm 0mm 0mm, clip]{./figures/treeAlg1.pdf}
		\caption{Initial partition with trivial parts assigned.}\label{sfig:treeAlg1}
	\end{subfigure}    \hfill
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[width=\textwidth,trim=0mm 0mm 0mm 0mm, clip]{./figures/treeAlg2.pdf}
		\caption{Merging monotone parts.}\label{sfig:treeAlg2}
	\end{subfigure}    \hfill
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[width=\textwidth,trim=0mm 0mm 0mm 0mm, clip]{./figures/treeAlg3.pdf}
		\caption{Merging reflective bitone parts.}\label{sfig:treeAlg3}
	\end{subfigure}
	\begin{subfigure}[b]{0.48\textwidth}
		\centering
		\includegraphics[width=\textwidth,trim=0mm 0mm 0mm 0mm, clip]{./figures/treeAlg4.pdf}
		\caption{Merging other bitone parts (output).}\label{sfig:treeAlg4}
	\end{subfigure}
	\caption{Our cluster aggregation algorithm on a unit-weight tree. The input partition $\mcV$ is blue and our output partition $\mcV'$ is red. \ref{sfig:treeAlg1} gives our input and initialization. \ref{sfig:treeAlg2} is the result from processing all monotone parts. \ref{sfig:treeAlg3} is the result of processing all bitone parts with a monotone down child. \ref{sfig:treeAlg4} is the result of processing all remaining bitone parts.}\label{fig:treeAlg}
\end{figure}

The following summarizes the properties of our algorithm.
\CATrees*
\begin{proof}
	We use the algorithm described above. The algorithm trivially runs in polynomial time. We begin by observing that this process is indeed a cluster aggregation solution in that $f(V_i)$ is a portal for every $V_i \in \mcV$. In particular, observe that each trivial, monotone and reflective bitone part is trivially assigned. The only remaining parts of $\mcV$ are those that are bitone but not reflective but any such $V_i$ must be such that the part containing $t_i'$ either is trivial, is monotone or is a reflective bitone part and so already assigned.
	
	Next, we analyze the distortion of the resulting cluster aggregation solution. As before we define the detour of $v$ as
	\begin{align*}
		\dtr_f(v) := d_{G[f(v)]}(v, P) - d_G(v, P).
	\end{align*}
	It will be convenient for our presentation to ignore distances inside of clusters with portals. Thus, we let $\tilde{\dtr}$ give the detour a vertex must travel to get to any vertex in a cluster containing a portal, namely
	\begin{align*}
		\tilde{\dtr}_f(v) := d_{G[f(v)]}(v, \tilde{P}) - d_G(v, \tilde{P}).
	\end{align*}
	Similarly, we let $\tilde{f}(v)$ be all vertices in the part of $\mcV$ containing $f(v)$. Observe that to show $\dtr_f(v)$ is at most $\beta \cdot \Delta $, it suffices to show that $\tilde{\dtr}_f(v) \leq (\beta - 1) \cdot \Delta$ since if $\tilde{\dtr}_f(v) \leq \beta - 1$ then we have
	\begin{align*}
		\dtr_f(v) & = d_{G[f(v)]}(v, P) - d_G(v, P)\\
		& \leq d_{G[f(v)]}(v, \tilde{P}) + \Delta - d_G(v, \tilde{P})\\
		& \leq \beta \cdot \Delta.
	\end{align*}
	Our goal is to show that $\dtr_f(v)$ is at most $5\Delta$ for every $v \in V$ and so it suffices to show $\tilde{\dtr}_f(v) \leq 4 \Delta$ for every $v$. 
	
	The intuition for showing that $\tilde{\dtr}_f(v) \leq 4 \Delta$ is as follows. Roots of monotone parts and vertices in trivial parts have  $\tilde{\dtr}$ value of $0$ by construction. On the other hand, non-root vertices of monotone parts must traverse their parts, potentially paying $\Delta$ for the distance travelled and another $\Delta$ for potentially increasing their distance to $\tilde{P}$ by $\Delta$ for a cumulative $\tilde{\dtr}$ value of $2\Delta$. Vertices in reflective bitone parts eventually get to a trivial part or a root of a monotone down part at which point they pay $\tilde{\dtr}$ value of $0$ but in order to get to this root they must incur $2 \Delta$ in $\tilde{\dtr}$, similarly to non-root vertices in monotone parts. Lastly, vertices in non-reflective bitone parts must pay $2 \Delta$ to eventually get to a reflective bitone part or monotone part at which point they pay the $2 \Delta$ for which this part already paid for $4 \Delta$ total.
	
	For the remainder of this proof we consider a fixed vertex $v$ in a part $V_i \in \mcV$ that does not contain a portal (the proof is trivial if $v_i$ contains a portal). We case on what type of part $V_i$ is.
	
	Suppose $V_i$ is trivial. Then $v \in \tilde{P}$ and so we trivially have $\tilde{\dtr}_f(v) = 0$.
	
	Suppose $V_i$ is monotone. If $V_i$ is monotone up we claim that $\tilde{\dtr}_f(v) \leq 2\Delta$ and, further, if $v = r_i$ we claim $\tilde{\dtr}_f(v) = 0$. Every cluster that $P_i$ intersects other than $V_j$ is also monotone up. It follows that to get to $\tilde{P}$ in $G[f(v)]$, $v$ may have to traverse its own cluster until it reaches $r_i$ at which point it can follow $P_i$ to $t_i$. Thus, since $d_G(v, r_i) \leq \Delta$ and $d_G(r_i, t_i) \leq d_G(v, \tilde{P}) + \Delta$, we get
	\begin{align*}
		d_{G[f(v)]}(v, \tilde{P}) &= d_G(v, r_i) + d_G(r_i, t_i)\\
		& \leq 2 \Delta + d_G(v, \tilde{P}),
	\end{align*}
	implying $\tilde{\dtr}_f(v) \leq 2\Delta$. Furthermore, observe that if $v = r_i$ then $d_G(v, r_i) = 0$ and $d_G(r_i, t_i) = d_G(v,\tilde{P})$ and so in this case we get $\tilde{\dtr}_f(v) = 0$. If $V_i$ is monotone down then a symmetric argument shows that $\tilde{\dtr}_f(v) \leq 2\Delta$ and $\tilde{\dtr}_f(v) = 0$ if $v = r_i$.
	
	% we claim $\dtr_f(v) \leq 2\Delta$. In particular, in this case $v$ to get to its portal in our cluster aggregation solution must first go to $r_i$, follow $P_i$ to $t_i \in V_j$ and then go to the portal $p_j$ in $V_j$. However, observe that the portal in $p_j$
	
	% Letting $P_i'$ be $P_i$ concatenated with the shortest path from $t_i$ to $p_j$ we have
	% \begin{align*}
	%     w(P_i') \leq d_G(v, P) + \Delta
	% \end{align*}
	% and so $\dtr_f(v) \leq 2\Delta$. A symmetric argument shows that $\dtr_f(v) \leq \Delta$ for every vertex in a monotone down part.
	
	Next, suppose $V_i$ is a reflective bitone part. We claim that in this case $\tilde{\dtr}_f(v) \leq 2\Delta$. Specifically, in this case in order to get to $\tilde{P}$, vertex $v$ must traverse $V_i$ until it reaches $r_j' \in V_i$ which is the parent of some $r_j \in V_j$ in $G$ where $V_j$ is either trivial or monotone down. Vertex $v$ then goes to $r_j$ and on to $\tilde{f}(V_j)$. However, observe that since $V_i$ is a reflective part we know
	\begin{align}\label{eq:af}
		w(\{r_j, r_j'\}) + d_G(r_j, \tilde{P}) = d_G(r_j', \tilde{P})
		% w(\{r_j, r_j'\}) + d_G(r_j, P) \leq w(\{r_j, r_j'\}) + d_G(r_j, \tilde{P}) + \Delta = d_G(r_j', \tilde{P}) +\Delta \leq d_G(r_j', P) + \Delta
	\end{align}
	
	
	Moreover $V_j$ must either be trivial or monotone down with root $r_j$ and so in either case we know that $\tilde{\dtr}_{f}(r_j) = 0$ and, in particular, 
	\begin{align}\label{eq:asf}
		d_G(r_j, \tilde{f}(V_j)) = d_G(r_j, \tilde{P}).
	\end{align}
	Combining Equations \ref{eq:af} and \ref{eq:asf} with the fact that $d_G(v, r_j') \leq \Delta$ and $d_G(r_j', \tilde{P}) \leq d_G(v, \tilde{P}) + \Delta$, overall we get
	\begin{align*}
		d_{G[f(v)]}(v, \tilde{P}) &= d_G(v, r_i') + w(\{r_j, r_j'\}) + d_G(r_j, \tilde{f}(V_j)) \\
		& \leq \Delta + w(\{r_j, r_j'\}) + d_G(r_j, \tilde{P})\\
		& = \Delta + d_G(r_j', \tilde{P})\\
		& \leq d_G(v, \tilde{P}) + 2\Delta,
	\end{align*}
	showing $\tilde{\dtr}_f(v) \leq 2\Delta$.
	
	Lastly, suppose $V_i$ is a bitone part that is not reflective. We claim $\tilde{\dtr}_f(v) \leq 4 \Delta$. In such a case in order to get to $\tilde{P}$, $v$ must first go to $r_i$ then continue along a path from $r_i$  to a vertex $t_i' \in V_j$ where $V_j$ is either a monotone part or a reflective bitone part and this path is a subpath of a shortest path from $r_i$ to $\tilde{P}$. Vertex $v$ must then traverse from $t_i'$ to $\tilde{f}(V_j)$. 
	
	Since $V_j$ is either a monotone part or a reflective bitone part, by the above argument we know that  $\tilde{\dtr}_f(t_i') \leq 2 \Delta$ and so $d_G(t_i', \tilde{f}(V_j)) \leq 2 \Delta + d_G(t_i', \tilde{P})$. Furthermore, $d_G(t_i', \tilde{P}) = d_G(r_i, \tilde{P}) - d_G(r_i, t_i') \leq \Delta + d_G(v, \tilde{P}) - d_G(r_i, t_i')$ and so
	%$d_G(t_i', P) = d_G(v, P) - d_G(v, t_i')$ and so
	\begin{align*}
		d_G(t_i', \tilde{f}(V_j)) \leq 3 \Delta + d_G(v, \tilde{P}) - d_G(r_i, t_i') \label{eq:acd}
	\end{align*}
	Thus, applying this inequality and the fact that $d_G(v, r_i) \leq \Delta$, we get that the total distance traveled by $v$ to $\tilde{P}$ is
	\begin{align*}
		d_{G[f(v)]}(v, \tilde{P}) & = d_G(v, r_i) + d_G(r_i, t_i') + d_G(t_i', \tilde{f}(V_j))\\
		& \leq  4 \Delta + d_G(v, \tilde{P}),
	\end{align*}
	showing $\tilde{\dtr}_f(v) \leq 4 \Delta$ as required.
\end{proof}

